Violation of chirality of the M\"obius domain-wall Dirac operator from the eigenmodes

We investigate the effects of the violation of the Ginsparg-Wilson (GW) relation in the M\"obius domain-wall fermion formulation on the lattice with finite fifth dimension. Using a decomposion in terms of the eigenmodes of its four-dimensional effective Dirac operator, we isolate the GW-violating terms for various physical quantities including the residual mass and the meson susceptibilities relevant for the effective restoration of the axial U(1) symmetry at finite temperature. Numerical result shows that the GW-violating effect is more significant, or even overwhelming, for the quantities that are dominated by the low-lying eigenmodes.

==> table_noratio.tex <==
      $\beta$ & $m$ & $N_s$ & $N_t$ & $L_s$ & $N_{\rm conf}$ & $N_{\rm ev}$ &$\langle \Delta_{\rm full} \rangle$   &$\langle \Delta_{\rm violation} \rangle$ & $\langle \Delta_{\rm stochastic}\rangle$ & $\langle \Delta_{\rm violation}\rangle/ \langle \Delta_{\rm full}\rangle$  \\\hline 
      4.07	&   0.01	&16&8&12&	239& 86&    0.1395 $\pm$ 0.0129 &	0.0527 $\pm$    0.0037      &         0.1404 $\pm$ 0.0131   &    0.378 $\pm$	0.026\\
      4.10	&   0.01        &16&8&12&	203& 86&    0.0641 $\pm$ 0.0115 &	0.0179 $\pm$    0.0028      &         0.0615 $\pm$ 0.0112   &    0.279 $\pm$    0.040   \\
      4.10	&   0.01        &32&8&12&        85& 48&    0.0687 $\pm$ 0.0053 &	0.0207 $\pm$    0.0015      &         0.0692 $\pm$ 0.0053   &    0.302 $\pm$    0.024   \\
      4.07	&   0.001       &16&8&24&	210& 69&    0.0497 $\pm$ 0.0141 &	0.0490 $\pm$    0.0138      &         0.0509 $\pm$ 0.0147   &    0.982 $\pm$    0.002      \\
      4.07	&   0.001       &32&8&24&	215& 25&    0.1055 $\pm$ 0.0351 &	0.0691 $\pm$    0.0169      &         0.1058 $\pm$ 0.0340   &    0.654 $\pm$    0.105      \\
      4.10	&   0.001       &16&8&24&	124& 84&    0.0233 $\pm$ 0.0131	&	0.0230 $\pm$	0.0129      &         0.0232 $\pm$ 0.0130   &    0.983 $\pm$    0.004      \\
      4.10	&   0.005       &32&8&24& 	 98& 28&    0.1071 $\pm$ 0.0148	&	0.0181 $\pm$	0.0026      &         0.1088 $\pm$ 0.0151   &    0.170 $\pm$    0.023   \\
      4.10	&   0.001       &32&8&24& 	 69& 36&    0.0124 $\pm$ 0.0049	&	0.0122 $\pm$	0.0047      &         0.0128 $\pm$ 0.0050   &    0.975 $\pm$    0.006   \\
      4.18	&   0.01        &32&8&12& 	 80& 48&    0.0019 $\pm$ 0.0006	&	0.0011 $\pm$	0.0003      &         0.0020 $\pm$ 0.0006   &    0.616 $\pm$    0.061  \\\hline
      4.18	&   0.01	&32&12&16&	 54& 15&    0.2000 $\pm$ 0.0054	&	0.0159 $\pm$	0.0011      &         0.2073 $\pm$ 0.0058   &    0.080 $\pm$    0.006   \\
      4.22	&   0.01	&32&12&16&	 50& 38&    0.1213 $\pm$ 0.0044	&	0.0064 $\pm$	0.0007      &         0.1189 $\pm$ 0.0047   &    0.053 $\pm$    0.006   \\
      4.23	&   0.01	&32&12&16&       94& 22&    0.1090 $\pm$ 0.0047	&	0.0042 $\pm$	0.0004      &         0.1099 $\pm$ 0.0055   &    0.038 $\pm$    0.004   \\
      4.23	&   0.005	&32&12&16&      176& 30&    0.1074 $\pm$ 0.0081	&       0.0089 $\pm$	0.0010      &         0.1086 $\pm$ 0.0085   &    0.083 $\pm$    0.009   \\
      4.23	&   0.0025	&32&12&16&       78& 24&    0.2162 $\pm$ 0.0414	&       0.0350 $\pm$	0.0071      &         0.2142 $\pm$ 0.0423   &    0.162 $\pm$    0.022      \\
      4.24	&   0.01	&32&12&16&	326& 38&    0.1016 $\pm$ 0.0031	&	0.0047 $\pm$	0.0003      &         0.1047 $\pm$ 0.0035   &    0.046 $\pm$    0.003   \\
      4.24	&   0.005	&32&12&16&       95& 33&    0.1246 $\pm$ 0.0133	&       0.0072 $\pm$	0.0014      &         0.1177 $\pm$ 0.0137   &    0.057 $\pm$    0.011\\
      4.24	&   0.0025	&32&12&16&      111& 39&    0.0416 $\pm$ 0.0133 &       0.0135 $\pm$	0.0041      &         0.0432 $\pm$ 0.0138   &    0.323 $\pm$    0.080  \\
      4.30	&   0.01	&32&12&16&      195& 38&    0.0447 $\pm$ 0.0028	&	0.0003 $\pm$	0.0001      &         0.0425 $\pm$ 0.0028   &    0.007 $\pm$    0.003\\


==> table_simple.tex <==
      $\beta$ & $m$ & $N_s$ & $N_t$ & $L_s$ & $N_{\rm conf}$ & $N_{\rm ev}$ &$\langle \Delta_{\rm violation}\rangle/ \langle \Delta_{\rm full}\rangle$  & $\langle \Delta_{\rm stochastic}\rangle/\langle \Delta_{\rm full}\rangle$ \\\hline 
      4.07	&   0.01	&16&8&12&	239& 86&    0.378 $\pm$	0.026	&	1.0015 $\pm$          0.0090    \\
      4.10	&   0.01        &16&8&12&	203& 86&    0.279 $\pm$ 0.040   &	0.9874 $\pm$          0.0117    \\
      4.10	&   0.01        &32&8&12&        85& 48&    0.302 $\pm$ 0.024   &	1.0074 $\pm$          0.0057    \\
      4.07	&   0.001       &16&8&24&	210& 69&    0.982 $\pm$ 0.002   &	1.0124 $\pm$          0.0198    \\
      4.07	&   0.001       &32&8&24&	215& 25&    0.654 $\pm$ 0.105   &	0.9979 $\pm$          0.0209    \\
      4.10	&   0.001       &16&8&24&	124& 84&    0.983 $\pm$	0.004	&	0.9937 $\pm$	      0.0162    \\
      4.10	&   0.005       &32&8&24& 	 98& 28&    0.170 $\pm$	0.023	&	1.0090 $\pm$	      0.0113    \\
      4.10	&   0.001       &32&8&24& 	 69& 36&    0.975 $\pm$	0.006	&	1.0220 $\pm$	      0.0108    \\
      4.18	&   0.01        &32&8&12& 	 80& 48&    0.616 $\pm$	0.061	&	1.0969 $\pm$	      0.0279    \\\hline
      4.18	&   0.01	&32&12&16&	 54& 15&    0.080 $\pm$	0.006	&	1.0126 $\pm$	      0.0043    \\
      4.22	&   0.01	&32&12&16&	 50& 38&    0.053 $\pm$	0.006	&	1.0051 $\pm$	      0.0069    \\
      4.23	&   0.01	&32&12&16&       94& 22&    0.038 $\pm$	0.004	&	1.0020 $\pm$	      0.0056    \\
      4.23	&   0.005	&32&12&16&      176& 30&    0.083 $\pm$	0.009	&       1.0054 $\pm$	      0.0064    \\
      4.23	&   0.0025	&32&12&16&       78& 24&    0.162 $\pm$	0.022	&       1.0028 $\pm$	      0.0119    \\
      4.24	&   0.01	&32&12&16&	326& 38&    0.046 $\pm$	0.003	&	1.0077 $\pm$	      0.0025    \\
      4.24	&   0.005	&32&12&16&       95& 33&    0.057 $\pm$	0.011	&       0.9883 $\pm$	      0.0077    \\
      4.24	&   0.0025	&32&12&16&      111& 39&    0.323 $\pm$	0.080   &       0.9995 $\pm$	      0.0214    \\
      4.30	&   0.01	&32&12&16&      195& 38&    0.007 $\pm$	0.003	&	1.0170 $\pm$	      0.0060    \\

